Fine-Tuning Language Models Using Formal Methods Feedback

Although pre-trained language models encode generic knowledge beneficial for planning and control, they may fail to generate appropriate control policies for domain-specific tasks. Existing fine-tuning methods use human feedback to address this limitation, however, sourcing human feedback is labor intensive and costly. We present a fully automated approach to fine-tune pre-trained language models for applications in autonomous systems, bridging the gap between generic knowledge and domain-specific requirements while reducing cost. The method synthesizes automaton-based controllers from pre-trained models guided by natural language task descriptions. These controllers are verifiable against independently provided specifications within a world model, which can be abstract or obtained from a high-fidelity simulator. Controllers with high compliance with the desired specifications receive higher ranks, guiding the iterative fine-tuning process. We provide quantitative evidences, primarily in autonomous driving, to demonstrate the method's effectiveness across multiple tasks. The results indicate an improvement in percentage of specifications satisfied by the controller from 60% to 90%.

==> sec/0-abstract.tex <==
\begin{abstract}


We present a novel, fully automated approach to enhance pre-trained language models for applications in autonomous systems, addressing the challenge of bridging the gap between generic knowledge and domain-specific requirements. Leveraging formal verification feedback, the method synthesizes automaton-based controllers from pre-trained models, guided by natural language task descriptions. These controllers are formally verifiable against specifications within a world model. Iterative fine-tuning using verification feedback ensures alignment with desired specifications. In scenarios where obtaining an accurate world model is challenging, empirical trajectories from high-fidelity simulators provide verification feedback. Controllers with high compliance receive higher ranks, guiding the fine-tuning process. Empirical studies, primarily in autonomous driving, demonstrate our approach's effectiveness across multiple tasks. Our approach yields outputs meeting a substantial portion of the specified criteria, and our synthesized controllers also demonstrates real-world applicability.

% Although LLM can do planning and control, they are limited for domain-specific tasks.
% Existing fine-tuning methods via human feedback are able to address this limination, however, collecting humna feedback is expensive and labor intensive.
% We propose a method that fine-tunes LLM via verification feedback to place human feedback, which reduces the labor intensive and cheaper, while resolving the domain specificity problem.
% Specifically,....
% We provide an alternative method to take account for the absence of the world model that encoding domain-specific knowledge. The method ...
% We provide empirical evidence to show... (no real world applicability)

\end{abstract}
\glsresetall

==> sec/1-introduction.tex <==
\section{Introduction}

% LLMs can be used for control in general
Pre-trained language models encompass a vast array of knowledge beneficial for both planning and control. 
Recent works use pre-trained models to synthesize control policies for autonomous systems such as in autonomous driving \cite{seff2023motionlm}, surgical robotics \cite{janssen2023use}, and aircraft operation \cite{aerospace10090770}. The control policies yield high-level actions that an agent should take in order to satisfy objectives specified via natural language prompts.
% LLMs may fail in specific domains because they lack domain specific knowledge
However, in specific domains, pre-trained models may fail to generate appropriate control policies. For instance, an autonomous driving system may require knowledge about traffic rules and conventions specific to a given country. Such specific rules and conventions may be beyond the knowledge encoded in the pre-trained model. 

% This problem may be addressed through multiple methods... Human feedback fails because domain specific knowledge is costly and labor intensive to acquire. 
To bridge this gap, many researchers have turned to human feedback to refine these models, ensuring they possess the necessary domain-specific knowledge \cite{RLHF, Christiano2017RLHF, Rafailov2023DPO}. Such feedback gauges how well a model's output aligns with set objectives. Simple feedback mechanisms, like binary rankings, can be instrumental and allow implicit incorporation of domain-specific knowledge. However, sourcing human feedback is both time-consuming and expensive.

%To address this shortcoming, several works use human feedback for fine-tuning pre-trained models and to incorporate required domain knowledge \cite{RLHF, Christiano2017RLHF, Rafailov2023DPO}. Human feedback evaluates the extent to which the output of a pre-trained model aligns with the desired objectives. For example, provision of a binary ranking of like or dislike for each model output can act as a feedback source. This feedback from human expertise enables fine-tuning of the pre-trained model and allows implicit incorporation of domain-specific knowledge. However, obtaining feedback from humans is labor intensive and costly.

% domain knowledge can also be expressed using formal methods, and we develop a method to use domain knowledge expressed as formal methods into LLMs. 
An alternative to human feedback is formal verification feedback. Given a world model and set of logical specifications, formal methods allow verification of compliance of the output of a given pre-trained model with these specifications. The world model may be abstract or derived directly from a high-fidelity simulator in certain domains. An output from the pre-trained model can be verified against the world model via logical specifications to ensure compliance with desired behavior. This measure of compliance can act as a source of feedback for fine-tuning similar to human feedback. Since this verification can be automated, formal verification feedback is less labour intensive and cheaper.


We present a novel approach for refining pre-trained models using formal verification feedback, aiming to enhance their performance in various natural language tasks. Our method leverages automaton-based controllers synthesized from the pre-trained model, guided by task descriptions in natural language. These controllers are designed to be formally verifiable against externally provided specifications when integrated into a specific world model. Our approach hinges on the use of formal verification to assess the extent to which each controller, derived from the pre-trained model, satisfies the specified requirements. We employ this verification feedback iteratively to fine-tune the pre-trained model until the synthesized controller aligns with the desired specifications.

In cases where acquiring an accurate world model is unfeasible, we acquire feedback through empirical evaluation, garnered from a high-fidelity simulator. This involves collecting observational data and corresponding control actions, forming a sequence of state-action pairs. Each sequence is rigorously verified against the provided specifications. Controllers that exhibit a high degree of compliance with these specifications when executed in the simulator are assigned higher ranks. Subsequently, these ranks are employed as a guiding metric for fine-tuning.

To assess the effectiveness of our proposed method, we conduct empirical studies across multiple tasks within the context of an autonomous driving system. However, it is important to note that the applicability of our approach extends beyond this domain. Our quantitative results underscore the efficacy of our method in refining pre-trained models, resulting in outputs that meet a substantial portion of the specified criteria. Additionally, we demonstrate the real-world applicability of controllers synthesized from the fine-tuned pre-trained model, thereby reinforcing the relevance and significance of our proposed approach.

The main strengths of our work are outlined as follows:

\begin{itemize}
    \item We introduce a novel approach that leverages formal verification to fine-tune pre-trained models, without any human intervention. It bridges the gap between generic knowledge and domain-specific requirements.
    % \item Our approach is adaptable to scenarios where acquiring a precise world model is challenging, by using empirical observations from simulators, making it particularly flexible in real-world applications.
    \item By using empirical observations from simulators, our approach is adaptable to scenarios where acquiring a precise world model is challenging,  making it particularly flexible in real-world applications.
    \item We demonstrate the versatility of the proposed method by conducting empirical studies in the domain of autonomous driving, showcasing its effectiveness across multiple tasks.
\end{itemize}





% Extra:
% Furthermore, given reliable visual observations and the fact that the synthesized policies from the LLM outputs are solely based on visual observations, the policies can transfer from simulation to real-world cases consistently with formal guarantees. Such sim-to-real transfer with formal guarantees, without the need for human feedback, strengthens the necessity of our approach, especially since violating safety-critical rules in reality, such as in autonomous driving, leads to serious consequences.
% The experimental results demonstrate this desired behavior and confirm the applicability of the proposed method.


% The main contribution of this paper is two-fold:
% \begin{itemize}
%     \item We develop a method that fine-tunes LLMs in an automated manner via formal verification feedback instead of human feedback.
%     % \item Due to the inherent formal method distillation, we generate control policies using LLMs that can be verified. 
%     \item Our method generates controllers that can directly operate in the real-world autonomous system with safety and task-satisfaction guarantees.
%     % \item We provide an approach to directly execute the control policies in the autonomous system due to the use of the models.
% \end{itemize}

